Actionable and Political Text Classification using Word Embeddings and LSTM

In this work, we apply word embeddings and neural networks with Long Short-Term Memory (LSTM) to text classification problems, where the classification criteria are decided by the context of the application. We examine two applications in particular. The first is that of Actionability, where we build models to classify social media messages from customers of service providers as Actionable or Non-Actionable. We build models for over 30 different languages for actionability, and most of the models achieve accuracy around 85%, with some reaching over 90% accuracy. We also show that using LSTM neural networks with word embeddings vastly outperform traditional techniques. Second, we explore classification of messages with respect to political leaning, where social media messages are classified as Democratic or Republican. The model is able to classify messages with a high accuracy of 87.57%. As part of our experiments, we vary different hyperparameters of the neural networks, and report the effect of such variation on the accuracy. These actionability models have been deployed to production and help company agents provide customer support by prioritizing which messages to respond to. The model for political leaning has been opened and made available for wider use.

==> texfiles/actionability_dl_model_evaluation.tex <==
% % Politician replies
% % Train on 795278 samples, validate on 198820 samples
% % Epoch 1/2
% % 795278/795278 [==============================] - 2253s - loss: 0.3096 - acc: 0.8583 - val_loss: 0.2847 - val_acc: 0.8694
% % Epoch 2/2
% % 795278/795278 [==============================] - 2275s - loss: 0.2625 - acc: 0.8822 - val_loss: 0.2812 - val_acc: 0.8706
% % 198820/198820 [==============================] - 110s     
% % Test score: 0.281173370393
% % Test accuracy: 0.870616638165

% % Dem v Rep
% % Train on 2174580 samples, validate on 543646 samples
% % Epoch 1/2
% % 2174580/2174580 [==============================] - 6268s - loss: 0.5702 - acc: 0.6967 - val_loss: 0.5508 - val_acc: 0.7111
% % Epoch 2/2
% % 2174580/2174580 [==============================] - 9890s - loss: 0.5355 - acc: 0.7231 - val_loss: 0.5407 - val_acc: 0.7185
% % 543646/543646 [==============================] - 673s     
% % Test score: 0.540693156996
% % Test accuracy: 0.718511678556

% % Only mentions
% % Train on 1975467 samples, validate on 493867 samples
% % Epoch 1/2
% % 1975467/1975467 [==============================] - 7317s - loss: 0.5611 - acc: 0.7057 - val_loss: 0.5404 - val_acc: 0.7210
% % Epoch 2/2
% % 1975467/1975467 [==============================] - 5747s - loss: 0.5232 - acc: 0.7331 - val_loss: 0.5286 - val_acc: 0.7292
% % 493867/493867 [==============================] - 278s     
% % Test score: 0.528586973831
% % Test accuracy: 0.729234793983



% % By lists
% % LSTM 128 units
% % X_train shape: (334713, 100)
% % X_test shape: (83679, 100)
% % Build model...
% % Train...
% % Train on 334713 samples, validate on 83679 samples
% % Epoch 1/3
% % 334713/334713 [==============================] - 1795s - loss: 0.5460 - acc: 0.7100 - val_loss: 0.5141 - val_acc: 0.7336
% % Epoch 2/3
% % 334713/334713 [==============================] - 1786s - loss: 0.4731 - acc: 0.7642 - val_loss: 0.5050 - val_acc: 0.7437
% % Epoch 3/3
% % 334713/334713 [==============================] - 1778s - loss: 0.4305 - acc: 0.7922 - val_loss: 0.5016 - val_acc: 0.7445
% % 83679/83679 [==============================] - 88s     
% % Test score: 0.501570215141
% % Test accuracy: 0.744499814768

% % LSTM 256 units
% % Train on 334713 samples, validate on 83679 samples
% % Epoch 1/2
% % 334713/334713 [==============================] - 660s - loss: 0.5434 - acc: 0.7113 - val_loss: 0.5067 - val_acc: 0.7391
% % Epoch 2/2
% % 334713/334713 [==============================] - 848s - loss: 0.4699 - acc: 0.7662 - val_loss: 0.4985 - val_acc: 0.7431
% % 83679/83679 [==============================] - 57s     
% % Test score: 0.498547833362
% % Test accuracy: 0.743125515362

% % LSTM 64 units
% \begin{table*}[!ht]
% \small
% \caption{LSTM models for Actionability}
% \centering
% \begin{tabular}{|l||r|r|r|r|r|r|}
%   \hline
%   \rowcolor{Gray} \parbox[t]{1.5cm}{\textbf{Model}} & \parbox[t]{1.5cm}{\textbf{Training Samples}} & \parbox[t]{1.5cm}{\textbf{Test Samples}} & \parbox[t]{1.5cm}{\textbf{Training (100k) \newline Accuracy}} & \parbox[t]{1.5cm}{\textbf{Test (100k) \newline Accuracy}} & \parbox[t]{1.5cm}{\textbf{Training (20k) \newline Accuracy}} & \parbox[t]{1.5cm}{\textbf{Test (20k) \newline Accuracy}}\\
%   \hline % \hhline{|=||=|=|}
%   % * - no punct     & 1,417,723 & 354,431   &   -    &   -    & 0.8802 & 0.8681 \\ \hline 
%   % * - with punct   & 1,417,723 & 354,431   & 0.9031 & 0.8597 &   -    &    -   \\ \hline 
%   af               & 174,119   & 43,530    & 0.8810 & 0.8525 & 0.8665 & 0.8547 \\ \hline
%   \rowcolor{red!50}
%   ar               & 380,038   & 95,010    & 0.8266 & 0.7940 & 0.8086 & 0.7950 \\ \hline
%   \rowcolor{green!50}
%   cs               & 31,407    & 7,852     & 0.9266 & 0.8988 & 0.9163 & 0.9087 \\ \hline
%   da               & 134,623   & 33,656    & 0.9098 & 0.8844 & 0.8974 & 0.8905 \\ \hline
%   de               & 223,438   & 55,860    & 0.8714 & 0.8316 & 0.8526 & 0.8352 \\ \hline
%   en               & 6,841,344 & 1,710,337 & 0.8540 & 0.8508 & 0.8490 & 0.8475 \\ \hline
%   es               & 720,783   & 180,196   & 0.8563 & 0.8406 & 0.8461 & 0.8402 \\ \hline
%   et               & 113,635   & 28,409    & 0.9140 & 0.8874 & 0.9050 & 0.8958 \\ \hline
%   \rowcolor{red!50}
%   fa               & 21,991    & 5,498     & 0.8308 & 0.7641 & 0.8160 & 0.7643 \\ \hline
%   \rowcolor{green!50}
%   fi               & 93,844    & 23,462    & 0.9247 & 0.8951 & 0.9103 & 0.9013 \\ \hline
%   fr               & 397,749   & 99,438    & 0.8349 & 0.8112 & 0.8197 & 0.8088 \\ \hline
%   hr               & 48,728    & 12,182    & 0.9166 & 0.8747 & 0.8976 & 0.8771 \\ \hline
%   hu               & 35,719    & 8,930     & 0.8251 & 0.8507 & 0.8814 & 0.8550 \\ \hline
%   id               & 403,060   & 100,766   & 0.8826 & 0.8624 & 0.8699 & 0.8616 \\ \hline
%   it               & 219,898   & 54,975    & 0.8915 & 0.8736 & 0.8818 & 0.8734 \\ \hline
%   lt               & 22,257    & 5,565     & 0.8655 & 0.8762 & 0.8803 & 0.8652 \\ \hline
%   nl               & 286,350   & 71,588    & 0.8530 & 0.8249 & 0.8361 & 0.8240 \\ \hline
%   no               & 140,932   & 35,234    & 0.9056 & 0.8798 & 0.8944 & 0.8843 \\ \hline
%   pl               & 79,386    & 19,847    & 0.9069 & 0.8668 & 0.8901 & 0.8787 \\ \hline
%   pt               & 465,925   & 116,482   & 0.8545 & 0.8357 & 0.8441 & 0.8363 \\ \hline
%   ro               & 81,920    & 20,481    & 0.9097 & 0.8726 & 0.8899 & 0.8798 \\ \hline
%   \rowcolor{green!50}
%   sk               & 73,808    & 18,452    & 0.9296 & 0.9000 & 0.9093 & 0.9098 \\ \hline
%   sl               & 76,784    & 19,196    & 0.9120 & 0.8658 & 0.8878 & 0.8728 \\ \hline
%   so               & 146,428   & 36,608    & 0.8911 & 0.8591 & 0.8773 & 0.8656 \\ \hline
%   sq               & 31,683    & 7,921     & 0.8991 & 0.8794 & 0.8846 & 0.8799 \\ \hline
%   \rowcolor{green!50}
%   sv               & 114,395   & 28,599    & 0.9276 & 0.9013 & 0.9151 & 0.9069 \\ \hline
%   sw               & 51,396    & 12,849    & 0.9029 & 0.8434 & 0.8778 & 0.8594 \\ \hline
%   \rowcolor{red!50}
%   th               & 52,859    & 13,215    & 0.8898 & 0.7601 & 0.8088 & 0.7997 \\ \hline
%   tl               & 356,072   & 89,018    & 0.8487 & 0.8253 & 0.8374 & 0.8261 \\ \hline
%   tr               & 123,217   & 30,805    & 0.8798 & 0.8291 & 0.8570 & 0.8331 \\ \hline
%   vi               & 58,769    & 14,693    & 0.8769 & 0.8542 & 0.8694 & 0.8541 \\ \hline
% \end{tabular}
% \label{table:lstm_model_acc}
% \end{table*}

% We perform several experiments on contextual classification of messages. 

% \subsection{Actionability}

% The first set of experiments is performed for the problem of actionability, where messages are classified as \textit{actionable} or \textit{non-actionable}.

% \subsubsection{Datasets}

% The research undertaken in this paper was performed on a social media management platform that helps agents respond to customer posts on behalf of their company.
% The platform prioritizes incoming messages from customers and routes them to the appropriate agents, and is integrated with major social networks, brand communities,
% and online forums. 
% Thus agents using the platform may respond to messages that are actionable, and ignore those that are not.
% If an agent provided a response, then the message is marked \textit{actionable}, otherwise it is marked \textit{non-actionable}.
% This labeled dataset is then used for training and evaluating models.

% In this study we used a trailing window of 6 months of data, from November 1st 2014 to May 1st 2015. 
% This included $46$ million unique messages, of which $0.7$ million were found to be actionable by agents. 
% All data analyzed here is publicly available on Twitter and Facebook and no private data was used as part of this research.

% Each message in the dataset has a "1" or "0" label, indicating whether the message was acted upon by an agent or not, respectively. 
% We create several train and test datasets.
% Equal number of actionable and non-actionable messages are sampled for each dataset. 
% The training and test datasets are created as 80/20 splits of the sampled data. 

% A pair of training and test datasets is created for each language, as well as one dataset that includes all languages. 

% The combined language dataset contains 1.7 million sampled messages across all languages. 

% \subsubsection{System Components}

% The system overview is shown in Figure \ref{figure:system_overview}.
% Data is ingested into the platform from social networks such as Twitter, Facebook and Google+, and messages are routed to company agents based on the mentioned company.
% The agent responses to the messages are recorded for each domain, which serves as the labeled data for model training and evaluation. 
% The collected public engagement data is written out to a Hadoop cluster that uses HDFS as the file system.
% We implement independent Java utilities with Hive UDF (User Defined Function) wrappers.

% \begin{figure}
%   \centering
%   \fbox{\includegraphics[width=0.97\columnwidth]{./figure/pdf/diagram/actionability_system_overview_large.pdf}}
%   \setlength{\abovecaptionskip}{0pt}
%   \caption{System Overview}
%   \label{figure:system_overview}
%   \vspace{-0.12in}
% \end{figure}

% \subsubsection{Multi-lingual contexts}

% We generate separate datasets for over 30 different languages and build models for each language. 
% Some languages have sparse data and smaller number of samples, while others are larger. 
% In our experiments dataset sizes varied from 27k messages for the language (Farsi) with the least data, to 8.5 million messages for the language with the most (English).

% We find from Table \ref{table:lstm_model_acc} that most languages show an accuracy of greater than 85\%.Languages such as Czech (cs), Finnish (fi), Slovak (si) and  Swedish (sv) show the highest accuracies of over 90\%. 
% The lowest accuracies are for languages such as Arabic (ar), Farsi (fa) and Thai (th), where the accuracies are slightly below 80\%. 
% Though in the case of fa and th, the low accuracy may be attributed to sparsity of data.

% We also generate a combined dataset of 1.7 million messages containing sampled data from all languages. 
% The model built using this dataset shows an accuracy of around 86\%. 
% Thus, a generalized model applicable across languages is able to capture actionability pretty well, though having a language specific model may give higher accuracies for some languages.

% \subsubsection{Vocabulary size}

% One of the parameters to consider while building models is the vocabulary size $V$. 
% The vocabulary used for training the models in each language is chosen by picking the top $V$ most frequent words seen in the corpus. 
% This parameter also determines the dimension of the feature space used for classification. 
% A higher dimension could presumably capture more information, at the cost of larger models ans slower training times.

% In our experiments we considered two vocabulary sizes for each language -- 20,000 and 100,000. 
% Table \ref{table:lstm_model_acc} shows the comparison of accuracies for the two vocabulary sizes.
% In general, we observe that there is little difference between the test accuracy values for the two vocabulary sizes.
% Thus even a smaller vocabulary is able to effectively capture actionability in messages, with the added advantage of faster training times. 

% \begin{table}[hbp]
% \small
% \setlength\tabcolsep{4pt}
% \caption{Language Performance}
% \centering
% \begin{tabular}{| l || p{2cm} | p{2cm} |}
%   \hline
%   \rowcolor{Gray} \textbf{Language} & \textbf{Traditional Model Accuracy} & \textbf{LSTM Accuracy} \\
%   \hline
%   \textbf{en} & 0.74 & 0.85 \\ \hline
%   \textbf{es} & 0.76 & 0.84 \\ \hline
%   \textbf{fr} & 0.76 & 0.81 \\ \hline
%   \textbf{pt} & 0.71 & 0.84 \\ \hline
%   \textbf{tl} & 0.79 & 0.83 \\ \hline
%   \textbf{id} & 0.74 & 0.86 \\ \hline
%   \textbf{af} & 0.75 & 0.85 \\ \hline
%   \textbf{it} & 0.72 & 0.87 \\ \hline
%   \textbf{nl} & 0.72 & 0.82 \\ \hline
%   \textbf{ar} & 0.81 & 0.80 \\ \hline
% \end{tabular}
% \label{table:language_performance}
% \end{table}

% \subsubsection{Comparison with Traditional Methods}

% In \cite{Spasojevic:actionability} we explored this problem through the lens of traditional supervised learning techniques. 
% Here we compare those results against the ones obtained by using the LSTM architecture. 

% We find from Table \cite{table:language_performance} that the LSTM models consistently outperform the best traditional supervised models for almost all the languages. 
% Only Arabic shows a slightly worse performance.
% Further the improvement is significantly large, the largest improvement being 15\% for Italian (it). 
% This clearly demonstrates the superiority of neural networks when it comes to the text classification problem of actionability.

% \subsubsection{Examples}

% \begin{table*}[!htp]
% \small
% \setlength\tabcolsep{4pt}
% \caption{Non-Actionable (NON) vs Actionable (ACT) Classification Examples}
% \centering
% \begin{tabular}{| p{10cm} | p{2cm} | p{2cm} |}
%   \hline
%   \rowcolor{Gray} \textbf{Message} & \textbf{Prediction Score} & \textbf{Classification} \\
%   \hline
% \rowcolor{green!50}
% @Verizon \#CEO confirms interest in possible @Yahoo acquisition & 0.02 & NON \\ \hline
% \rowcolor{green!40}
% @PGE4Me's new program allows customers to go 100\% \#solar without having to install rooftop solar panels! & 0.14 & NON \\ \hline 
% \rowcolor{green!30}
% Just another reason to despise @comcast and @xfinity Report: Comcast wants to limit Netflix binges & 0.15 & NON \\ \hline
% \rowcolor{green!20}
% We're switching up the Official 1D @Spotify Playlist, which classic tracks do you want to see added? & 0.32 & NON \\ \hline
% \rowcolor{green!10}
% I freaking HATE the changes @Yahoo has done to both the home page and my freaking mail!!! & 0.35 & NON \\ \hline 
% \rowcolor{orange!10}
% Thanks for the 6 hour outage in my area @comcast ill def be calling and having money taken off my monthly bill. & 0.59 & ACT \\ \hline
% \rowcolor{orange!20}
% @PGE4Me what's up with your online portal?  Taking forever to login and then everything says unavailable & 0.73 & ACT \\ \hline
% \rowcolor{orange!30}
% % Hey @Comcast why is my internet speed 84mbps down 23mbps up when I pay for 105mbps in Chicago? @ComcastCares @xfinity #comcast #speedtest & 0.74 & ACT \\ \hline
% @comcastcares @XFINITY Help! My wife just bought an episode of a show that we already watched (for free). Can I reverse the charge? & 0.82 & ACT \\ \hline
% \rowcolor{orange!40} 
% @Yahoo I accidentally deleted my email, how do I get it back? & 0.85 & ACT \\ \hline 
% % Dear @Yahoo I am VERY upset that I cannot attain my password and am receiving NO help from you guys after weeks of trying & 0.86 & ACT \\ \hline 
% \rowcolor{orange!50}
% @SpotifyCares hi someone has hacked my spotify and it won't let me listen to music because they are listening from another device help :( & 0.96 & ACT \\ \hline
% \end{tabular}
% \label{table:actionability_examples}
% \end{table*}

% \subsection{Political Leaning}

% The second text classification problem we address is that of political leaning with respect to politics in the United States. 
% In this problem, we would like to classify messages as "Democratic" or "Republican", based on the views expressed in the message.

% \subsubsection{Dataset}

% For this problem, we build the training and test datasets as follows.
% First we pick users on Twitter whose political leanings are known. 
% We do this by using Twitter Lists, which are manually curated lists of users by other users of the social media platform.
% For the users on these lists we aggregate the messages that they posted over a period of $x$ months, between ddmmyy1 to ddmmyy2.
% The messages posted by the known Democrats as per the Lists are labeled '$0$', and those by known Republicans are labeled '$1$'.
% We then divide this dataset into the training and test sets with an 80/20 percent split.
% The training set contains $334,713$ messages and the test set contains $83,679$ messages. 

% To test the hypothesis that a larger dataset would enable a better model to be learnt, we also create another dataset for the same set of users over a larger time period (?).
% This dataset contains $3,311,096$ messages in the training set and $827,774$ in the test set.

% The list of users whose messages were aggregated, along with their known political leaning is available here []. 

% \subsubsection{Training and Evaluation}

% For training the model, we use a similar architecture as the one used for the actionability problem above, with 128 units each in the embedding and LSTM layers.
% The model achieves a $76.42$\% accuracy on the training set, and a $74.37$\% accuracy on the test set.

% We examine the effects of changing various params on the accuracy of the model.

% \begin{itemize}
% \item \textbf{Dataset size}: We found that training with the second dataset, which was 10 times larger than the first dataset did not significantly affect the accuracy of the model. In fact the accuracy fell slightly to $73.79$\% on the test set.

% \item \textbf{Batch size}: Experimenting with different batch sizes such as 32 and 64 did not lead to a significant change in the accuracy values. The advantage of training with a larger batch size was faster convergence.

% \item \textbf{Embedding Layer Units}: For a fixed number of units in the LSTM layer (64), changing the number of units in the Embedding layer shows a small increase in accuracy with increasing units.
% This is somewhat expected, since projecting the input into a higher dimensional vector space via the Embedding layer presumably allows for more distinguishing features to be picked up by the LSTM layer.
% Figure shows this graphically.

% \item \textbf{LSTM Layer Units}: When the Embedding layer is held fixed at 128 units, changing the number of units in the LSTM layer does not show a pronounced increasing or decreasing pattern. The best performance is achieved when the LSTM layer has 512 units, although a similar performance is observed for 128 units. 
% This line of inquiry requires further investigation into the factors that determine the optimal number of units in the LSTM layer for a known input size. 

% \item \textbf{Embedding and LSTM Layer Units}: When the Embedding and LSTM layers have the same number of units, larger sizes show higher accuracies, but the difference is nevertheless small. For example, using embedding and LSTM layers of 64 units each showed an accuracy of $73.72$\%  as compared to networks with layers of 256 units, which showed an accuracy of $74.31$\%. 

% \item \textbf{Optimizers}: Among the tested optimizers, the 'Adam' optimizer performs the best with and accuracy of $74.45$\%, followed by Adagrad with $73.67$\%. The 'Adamax' and 'RMSprop' optimizers showed similar performance with an accuracy of $72.42$\%.
% \item \textbf{Activation}: Finally, we observed the performance when the activation function was changed. The sigmoid activation performed slightly better than the tanh activation, with a difference of $0.6$\% in the accuracy.
% \end{itemize}

% \begin{figure*}[!htbp]
%   \centering
%   \fbox{\includegraphics[width=0.9\textwidth,height=8cm]{./figure/png/lstm_embed.png}}
%   \setlength{\abovecaptionskip}{0pt}
%   \caption{Accuracy vs LSTM and Embedding Layer Units}
%   \label{figure:acc_vs_units}
% \end{figure*}


% % LSTM - 64
% % 16 -  73.61
% % 32 -  73.65
% % 64 -  73.72 
% % 128 - 74.17
% % 256 - 74.31
% % 512 - 74.56

% % Embedding 128 
% % 16  - 74.10
% % 32  - 74.27
% % 64  - 74.17
% % 128 - 74.45 
% % 256 - 74.20
% % 512 - 74.52

% % Embedding = LSTM
% % 16  - 73.46
% % 32  - 73.87
% % 64  - 73.72
% % 128 - 74.45 
% % 256 - 74.31
% % 512 - 74.55

% % optimizers 
% % Adam - 74.45
% % RMSprop - 72.43
% % Adagrad - 73.67 
% % sgd - 53.00
% % Adamax - 72.41


% % experiments with different optimizers

% Thus, our experiments suggests that at the cost of a negligible loss in accuracy, smaller models are able to effectively classify political leaning, with the advantage of being able to train such models faster.
% The model built with 128 units each in the embedding and LSTM layers, trained with sigmoid activation and the Adam optimizer is available here [] for download. This model was built on the smaller dataset described above.  

% \subsubsection{Examples}

% An interesting aspect of the predictions made with the model, is that along with the final classification, the score for a given message is indicative of the strength of the prediction. 
% Thus a message with a score of 0.9 may express a strongly Republican view, whereas that with a score of 0.55 may be a more moderate message.
% Table \ref{} shows examples of predictions made by the model.

% \begin{table*}[ht]
% \small
% \setlength\tabcolsep{4pt}
% \caption{Democrat (DEM) vs Republican (REP) Classification Examples}
% \centering
% \begin{tabular}{| p{10cm} | p{2cm} | p{2cm} |}
%   \hline
%   \rowcolor{Gray} \textbf{Message} & \textbf{Prediction Score} & \textbf{Classification} \\
%   \hline
%   \rowcolor{blue!50}
%   % \#OregonStandoff has actually been a good example to use by advocates for upgrading U.S. education, mental healthcare, and \#Gunsense standards & 0.09 & DEM \\ \hline
%   Climate change is real and caused by human activity.Our job is to aggressively transform our energy system away from fossil fuels. & 0.10 & DEM \\ \hline
%   \rowcolor{blue!50}
%   The contrast between @HillaryClinton's depth of foreign policy knowledge and experience with this gang is astonishing. \#imwithher \#GOPDebate & 0.09 & DEM \\ \hline
%   \rowcolor{blue!40}
%   Beyonce proudly displayed black power and they all collectively displayed LGBT love, the conservatives are seething  & 0.14 & DEM \\ \hline
%   % The GOP are Doing Everything They Can to Take Your Vote Away. Every Progressive That Doesn't Vote Makes Their Job Easier. & 0.15 & DEM \\ \hline
%   \rowcolor{blue!40}
%   Obama's super progressive budget would pour billions into clean energy, Medicaid, and edu while raising taxes & 0.23 & DEM \\ \hline
%   \rowcolor{blue!30}
%   On our worst days, it's fair to say we are 100 times better than any Republican candidate. & 0.28 & DEM \\ \hline
%   \rowcolor{blue!30}
%   Both Hilary and Bernie mention climate change, the GOP...nothing. One of the biggest issues facing everyone, esp rural states who grow food. & 0.31 & DEM \\ \hline
%   \rowcolor{blue!20}
%   @POTUS's FY 2017 Budget makes smart investments in tackling \#climatechange, accelerating innovation, making Americans safer. & 0.39 & DEM \\ \hline
%   \rowcolor{blue!10}
%   America's opportunity gap is not just about economic inequality. It is also about racial inequality, and we need to tackle both together. & 0.43 & DEM \\ \hline
%   \rowcolor{red!10}
%   Kansas oil producers are receiving less than \$25/barrel and Obama wants \$10 of it for his radical agenda. \#TCOT \#budget & 0.57 & REP \\ \hline
%   \rowcolor{red!20}
%   THERE GOES FREEDOM: Twitter bans even MORE conservative accounts just for questioning Islam's attrocities! \#WakeUpAmerica \#1A & 0.68 & REP \\ \hline
%   \rowcolor{red!30}
%   We will stop heroin and other drugs from coming into New Hampshire from our open southern border. We will build a WALL and have security. & 0.76 & REP \\ \hline
%   \rowcolor{red!35}
%   Is Obama clueless about Radical Islam? Nope he knows exactly what they are doing and he supports it \#RedNationRising  & 0.80 & REP \\ \hline
%   \rowcolor{red!45}
%   750 Billion has been paid out to illegal immigrants per Fox, under Obamacare subsidies! That is wrong!! Deport them all. Go Trump. & 0.86 & REP \\ \hline
%   \rowcolor{red!45}
%   Veterans come before illegals, refugees, able-bodied welfare recipients - period. WAKE UP \#GOP \#WakeUpAmerica & 0.86 & REP \\ \hline
%   \rowcolor{red!60}
%   Between Obama, ISIS, Congress, welfare leaches, unfettered immigration and Liberalism this country has gone downhill fast. & 0.94 & REP \\ \hline
%   \rowcolor{red!60}
%   RETWEET if you agree: Obama's \#MosqueVisit shows he underestimates the threat of radical Islam! & 0.94 & REP \\ \hline
% \end{tabular}
% \label{table:demvrep_examples}
% \end{table*}


